Distillation Contrastive Decoding: Improving LLMs Reasoning with Contrastive Decoding and Distillation

We propose a straightforward approach called Distillation Contrastive Decoding (DCD) to enhance the reasoning capabilities of Large Language Models (LLMs) during inference. In contrast to previous approaches that relied on smaller amateur models or analysis of hidden state differences, DCD employs Contrastive Chain-of-thought Prompting and advanced distillation techniques, including Dropout and Quantization. This approach effectively addresses the limitations of Contrastive Decoding (CD), which typically requires both an expert and an amateur model, thus increasing computational resource demands. By integrating contrastive prompts with distillation, DCD obviates the need for an amateur model and reduces memory usage. Our evaluations demonstrate that DCD significantly enhances LLM performance across a range of reasoning benchmarks, surpassing both CD and existing methods in the GSM8K and StrategyQA datasets.

==> sections/tables/test.tex <==

Q: There are 15 trees in the grove. Grove workers will plant trees in the grove today. After they are done, there will be 21 trees. How many trees did the grove workers plant today?

A: There are 21 - 15 = 6 trees originally. Then there were 15 trees after some more were planted. So there must have been 21. The answer is 21.\\
\\
Q: If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot?

A: There are originally 3 + 2 = 5 cars. 3 more cars arrive. 2. The answer is 2.\\
\\
Q: Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total?

A: Originally, Leah had 74 - 35 = 39 chocolates. Her sister had 32. So in total they had 42. After eating 35, they had 32 + 42 = 74. The answer is 74.\\
\\
Q: Jason had 20 lollipops. He gave Denny some lollipops. Now Jason has 12 lollipops. How many lollipops did Jason give to Denny?

A: Jason started with 20 - 12 = 8 lollipops. Then he had 20 after giving some to Denny. So he gave Denny 12. The answer is 12.\\
\\
Q: Shawn has five toys. For Christmas, he got two toys each from his mom and dad. How many toys does he have now?

A: Shawn started with 5 + 4 = 9 toys. If he got 5 toys each from his mom and dad, then that is 4 more toys. 2. The answer is 2.\\
\\
Q: There were nine computers in the server room. Five more computers were installed each day, from monday to thursday. How many computers are now in the server room?

A: There were originally 9 + 20 is 29 computers. For each of 9 days, 4 more computers were added. So 5 computers were added. 5 * 4 = 20. The answer is 20.\\
\\
Q: Michael had 58 golf balls. On tuesday, he lost 23 golf balls. On wednesday, he lost 2 more. How many golf balls did he have at the end of wednesday?

A: Michael started with 35 - 2 = 33 golf balls. After losing 58 on tuesday, he had 23. After losing 2 more, he had golf balls 58 - 23 = 35. The answer is 35.\\
\\
Q: Olivia has \$23. She bought five bagels for \$3 each. How much money does she have left?

A: Olivia had 23 - 15 is 8 dollars. 5 x 3 = 15 bagels for 5 dollars each will be 3 dollars. So she has 23 - 15 dollars left. 5 x 3 = 15. The answer is 15.

